Speech Quality Assessment through MOS using Non-Matching References

Human judgments obtained through Mean Opinion Scores (MOS) are the most reliable way to assess the quality of speech signals. However, several recent attempts to automatically estimate MOS using deep learning approaches lack robustness and generalization capabilities, limiting their use in real-world applications. In this work, we present a novel framework, NORESQA-MOS, for estimating the MOS of a speech signal. Unlike prior works, our approach uses non-matching references as a form of conditioning to ground the MOS estimation by neural networks. We show that NORESQA-MOS provides better generalization and more robust MOS estimation than previous state-of-the-art methods such as DNSMOS and NISQA, even though we use a smaller training set. Moreover, we also show that our generic framework can be combined with other learning methods such as self-supervised learning and can further supplement the benefits from these methods.

==> 02-background.tex <==
\section{Related Work}
\label{sec:format}

\subsection{Full-reference and no-reference frameworks}

% MAY REMOVE THIS DUE TO SPACE CONSTRAINTS. WE ARE COVERING ALL RELATED WORKS IN INTRO. 



Full-reference measures includes methods like \PESQ~\cite{rix2001perceptual}, \POLQA~\cite{beerends2013perceptual}, \VISQOL~\cite{hines2015visqol}, \DPAM~\cite{manocha2020differentiable} and \CDPAM~\cite{manocha2021cdpam}. Although quite useful, they suffer from two critical drawbacks. First, the requirement of a paired clean reference for SQA limits their applicability in scenarios where the paired clean reference is not available. Second, these methods are sensitive to perceptually invariant transformations~\cite{manjunath2009limitations,al2020correlation}.

In contrast, no-reference measures (\eg\ \DNSMOS~\cite{reddy2020dnsmos}, \NISQA~\cite{mittag2021nisqa}, \SQAPP~\cite{Manocha:2022:SNS}, and MetricNet~\cite{yu2021metricnet}) perform well in scenarios where a clean reference is not available. However, these metrics: (i)~fail to generalize to unseen perturbations; (ii)~depend on an implicit clean reference that can be highly varying~\cite{manocha2021noresqa}, and (iii)~contain substantial label noise from human annotations~\cite{reddy2020dnsmos}.
%
% To address a few concerns, researchers proposed using non-matching references~\cite{manocha2021noresqa} instead to increase robustness. However, it relies on conventional metrics like SNR and SI-SDR that may not directly correlate with quality.


% \section{Related Works}
% \label{sec:background}

% \subsection{Full-reference and no-reference frameworks}

% The objective assessment of speech quality can be divided
% into two ways, intrusive and non-intrusive, depending on whether the clean reference exists. This includes methods like \PESQ~\cite{rix2001perceptual}, \POLQA~\cite{beerends2013perceptual}, \VISQOL~\cite{hines2015visqol}, \DPAM~\cite{manocha2020differentiable} and \CDPAM~\cite{manocha2021cdpam}. Although they are considered more accurate as they provide a higher correlation with subjective evaluations, they suffer from two critical drawbacks. First, the requirement of a paired clean reference for quality assessment limits their applicability to real-world scenarios as the paired clean reference is likely not available in those cases. Second, these methods have acknowledged shortcomings such as sensitivity to perceptually invariant transformations~\cite{hines2013robustness,manjunath2009limitations}, therefore hindering stability in more diverse tasks such as speech enhancement.

% In contrast, non-intrusive (distance) measurements use only the corrupted speech signal for quality assessment. This includes methods like \DNSMOS~\cite{reddy2020dnsmos}, \NISQA~\cite{mittag2021nisqa}, \SQAPP~\cite{Manocha:2022:SNS}, and MetricNet~\cite{yu2021metricnet}. These performs like human beings, forming a mapping from the perceived speech utterance to a quality score. They also suffer from various drawbacks including dependence on implicit clean reference that can be highly varying due to factors like mood and past experiences~\cite{manocha2021noresqa}, as well as substantial label noise from human annotations~\cite{reddy2020dnsmos}. Moreover, these metrics also fail to generalize to unseen noise types~\cite{dong2019classification}. 

% Also add in detail about the disadvantages of NORESQA framework.

\subsection{Non-matching reference frameworks}
\label{sec:nmr}


To address a few concerns, researchers proposed using non-matching references instead to increase robustness. It pointed out that the lack of generalization of no-reference metrics could be due to the formulation, wherein \emph{no} reference was provided to the model. To address these concerns, the paper proposed a non-matching reference framework \NORESQA~\cite{manocha2021noresqa} that was motivated by humans ability to assess quality independently of the speech content, and the ease of predicting relative scores rather than absolute ratings. However, it relies on conventional quality metrics like SNR and Si-SDR that may not directly correlate with quality. 
%To the best of our knowledge, no prior method has used a non-matching reference framework to predict relative MOS scores.


% However, it relies on conventional metrics like SNR and SI-SDR that may not directly correlate with quality.

% \NORESQA\cite{manocha2021noresqa} was recently released that pointed out that the lack of generalization of no-reference metrics was due to the formulation, wherein \emph{no} reference was provided to the models.
% %This is because these metrics learn an implicit distribution of clean references, which suffers from both~(a) high variance due to factors like mood and past experience, and~(b) substantial label variance from human annotations~\cite{reddy2020dnsmos}. 
% To ameliorate these concerns, a non-matching reference framework \NORESQA\ was proposed that was motivated by humans ability to assess quality independently of the speech content, as well as the ease of predicting relative scores rather than absolute ratings. However, it relies on conventional metrics like SNR and Si-SDR that may not directly correlate with quality. To the best of our knowledge, no prior method has used a non-matching reference framework to predict relative MOS scores.





==> README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> ablations.tex <==
\begin{table*}[t!]

\vspace{-0.25in}
\centering
\resizebox{\textwidth}{!}{
 \begin{tabular}{l l c c c c c c c c c c c c c c c}
 \toprule
  \multirow{2}{*}{\bf Type} & \multirow{2}{*}{\bf Name} & \multicolumn{3}{c}{\bf HiFiGAN~\cite{su2020hifi}} & \multicolumn{3}{c}{\bf VoCo~\cite{jin2017voco}}& \multicolumn{3}{c}{\bf FFTnet~\cite{jin2018fftnet}}& 
 \multicolumn{3}{c}{\bf BWE~\cite{feng2019learning}} & 
 \multicolumn{3}{c}{\bf Dereverb~\cite{su2019perceptually}} \\
 \cmidrule(lr){3-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11} \cmidrule(lr){12-14} \cmidrule(lr){15-17} 
 & &\bf MSE $\downarrow$ &\bf PC$\uparrow$ &\bf SC$\uparrow$ &\bf MSE$\downarrow$ &  \bf PC$\uparrow$ & \bf SC$\uparrow$ &\bf MSE$\downarrow$ & \bf PC$\uparrow$ & \bf SC$\uparrow$ &\bf MSE$\downarrow$ & \bf PC$\uparrow$ & \bf SC$\uparrow$ &\bf MSE$\downarrow$ & \bf PC$\uparrow$ & \bf SC$\uparrow$ \\
 \cmidrule(lr){1-17}
 
 
 \multirow{2}{*}{\bf Non-Int.}
  & {\bf DNSMOS} & 0.64 & 0.64 & 0.63 & 0.88 & 0.30 & 0.27 & 0.41 & 0.40 & 0.41 & 1.72 & 0.32 & 0.34 & 2.53 & 0.41 & 0.50 \\
  & {\bf NISQA} & 0.85 & 0.66 & 0.67 & 1.83 & 0.30 & 0.23 & 0.92 & 0.37 & 0.25 & 2.63 & 0.35 & 0.36 & 2.24 & 0.59 & 0.60 \\
 
  \cdashline{1-17}
  
  \multirow{3}{*}{\bf Abs. MOS}
  & {\bf Scratch} & 1.02 & -0.01 & 0.19 & 1.57 & 0.08 & 0.12 & 0.49 & -0.02 & -0.01 & 1.74 & 0.10 & 0.11 & 2.79 & 0.02 & 0.01 \\
  & {\bf SSL-small} & 0.88 & 0.47 & 0.47 & 1.05 & 0.05 & 0.15 & 0.97 & 0.22 & 0.23 & 1.25 & 0.25 & 0.10 & 1.32 & 0.25 & 0.36 \\
  & {\bf SSL-big} & 0.84 & 0.50 & 0.51 & 2.45 & 0.12 & 0.11 & 2.24 & 0.08 & 0.14 & 2.57 & -0.02 & -0.02 & 3.24 & -0.01 & 0.1 \\
  
 \cdashline{1-17}
 
 \multirow{3}{*}{\bf \OURS\,}
 & {\bf Scratch} & 0.79 & 0.06 & 0.10 & 0.99 & 0.38 & 0.27 & 0.31 & 0.01 & 0.02 & 0.59 & 0.12 & 0.21 & 1.43 & 0.14 & 0.13 \\
 & {\bf SSL-small} & 0.65 & 0.65 & 0.65 & 0.89 & 0.32 & 0.20 & 0.72 & 0.36 & 0.36 & 1.21 & 0.07 & 0.28 & 1.09 & 0.29 & 0.41 \\
 & {\bf SSL-big} & 0.70 & 0.63 & 0.62 & 1.05 & 0.26 & 0.12 & 0.50 & 0.51 & 0.48 & 1.96 & 0.28 & 0.19 & 0.94 & 0.10 & 0.10 \\
 \bottomrule
\end{tabular}
}
\caption{\textbf{Ablations - utterance level correlations (1)}: for \frameworkname\,, DNSMOS, NISQA and NORESQA-MOS. Mean Square Error (MSE), Spearman (SC), Pearson (PC) correlations are shown. All unpaired \frameworkname\, are obtained using $n=100$ NMRs. $\uparrow$ is better.}
\label{ablations_1}
\end{table*}
